Generator-Refiner-Examiner: A Tri-Module Data Augmentation Framework for 3D Human Avatar Learning from Monocular Videos

This paper addresses the challenge of reconstructing photorealistic and animatable 3D human avatars from monocular videos. While existing methods rely on combining per-subject optimization with generic human priors, they often fail to capture fine-grained details when training frames are limited. To mitigate this data scarcity, we propose TrioMan, a systematic tri-module framework for augmented 3D avatar learning. Our approach comprises three synergistic components. The Generator creates diverse unseen samples by imposing Gaussian perturbations on pose and camera. The Refiner improves the quality of generated data through one-step diffusion guided by texture and geometry cues. The Examiner selects subject-consistent samples using a dual-branch attention-based similarity evaluation. Experiments on the X-Humans and NeuMan benchmarks show that TrioMan outperforms state-of-the-art methods.

==> 0_abstract.tex <==
\begin{abstract}




% This paper focuses on reconstructing photorealistic and animatable 3D human avatars from captured monocular video. However, the inherent limitation, only a narrow range of poses and viewpoints availble, greatly restrict the model's ability to handle unseen scenarios. Existing methods either rely on per-subject optimization with limited pose samples or adopt general human priors, failing to directly take with the lack of subject-specific details. To the end, we propose TrioMan, a tri-module augmented framework tailored for 3D human avatar learning. This framework systematically addresses data scarcity through three complementary modules: the Generator, which synthesizes diverse unseen training data through Gaussian-distributed pose and camera perturbations; the Refiner, which enhances synthetic-real consistency using one-step diffusion with texture and geometry conditioning; and the Examiner, which selects high-fidelity samples via a dual-branch attention-based similarity evaluation. Extensive experiments on the X-Humans and NeuMan benchmark datasets demonstrate that our method outperforms state-of-the-art approaches.




% The core challenge lies in monocular inputs’ intrinsic data scarcity—they capture just a narrow range of poses and viewpoints, greatly restricting the model’s ability to handle unseen ones. Existing methods either rely on per-subject optimization with limited pose samples or adopt general human priors, failing to fundamentally resolve the key issue of subject-specific details insufficient. 

% This paper focuses on reconstructing photorealistic and animatable 3D human avatars from captured monocular videos. However, the inherent limitation of having only a narrow range of poses and viewpoints available greatly restricts the model's ability to handle unseen scenarios. Existing methods either rely on per-subject optimization with limited pose samples or adopt general human priors, both of which fail to directly address the fundamental scarcity of subject-specific details. To address this issue, we propose TrioMan, a tri-module augmented framework designed for 3D human avatar learning. This framework systematically tackles data scarcity through three complementary modules: (1) the Generator, which synthesizes diverse unseen training data using Gaussian-distributed pose and camera perturbations; (2) the Refiner, which enhances synthetic-real consistency through one-step diffusion with texture and geometry conditioning; and (3) the Examiner, which selects high-fidelity samples via a dual-branch attention-based similarity evaluation. Extensive experiments on the X-Humans and NeuMan benchmark datasets demonstrate that our method outperforms state-of-the-art approaches.

This paper aims to address the task of reconstructing photorealistic and animatable 3D human avatars from monocular videos. The main challenge is the limited range of poses and viewpoints in captured data, which reduces the model’s ability to generalize to unseen scenarios. 
Existing methods often rely on per-subject optimization or generic human priors. Both approaches fail to preserve subject-specific details when personalized training data are scarce.
To address the data scarcity issue, we propose TrioMan, a tri-module data augmentation framework for 3D human avatar learning. It tackles data scarcity through three complementary modules. The Generator creates diverse unseen samples by imposing Gaussian perturbations on pose and camera. The Refiner improves the quality of generated data through one-step diffusion guided by texture and geometry cues. The Examiner selects subject-consistent samples using a dual-branch attention-based similarity evaluation. Experiments on the X-Humans and NeuMan benchmarks show that TrioMan outperforms state-of-the-art methods.



\end{abstract}
